Implicit Incorporation of Heuristics in MPC-Based Control of a Hydrogen Plant

The replacement of fossil fuels in combination with an increasing share of renewable energy sources leads to an increased focus on decentralized microgrids. One option is the local production of green hydrogen in combination with fuel cell vehicles (FCVs). In this paper, we develop a control strategy based on Model Predictive Control (MPC) for an energy management system (EMS) of a hydrogen plant, which is currently under installation in Offenbach, Germany. The plant includes an electrolyzer, a compressor, a low pressure storage tank, and six medium pressure storage tanks with complex heuristic physical coupling during the filling and extraction of hydrogen. Since these heuristics are too complex to be incorporated into the optimal control problem (OCP) explicitly, we propose a novel approach to do so implicitly. First, the MPC is executed without considering them. Then, the so-called allocator uses a heuristic model (of arbitrary complexity) to verify whether the MPC's plan is valid. If not, it introduces additional constraints to the MPC's OCP to implicitly respect the tanks' pressure levels. The MPC is executed again and the new plan is applied to the plant. Simulation results with real-world measurement data of the facility's energy management and realistic fueling scenarios show its advantages over rule-based control.

==> inc/xx_ocp.tex <==
\section{Optimal Control Problem}
Main dynamics (\textit{without heating from H2}): 

\begin{IEEEeqnarray}{rCl}
	\mlp\kpo & = & \mlp\k + \left( \mdotely\k - \mdotlpmp\k \right) \cdot \Tsampk \label{eq:dyn_lp} \\
	\mmp\kpo & = & \mmp\k + \left( \mdotlpmp\k - \mdotfuelmp\k \right) \cdot \Tsampk \label{eq:dyn_mp}
\end{IEEEeqnarray}

Balance Equation: 
\begin{IEEEeqnarray}{rCl}
	\Pgrid\k + \Pdemk + \Ppv\k - (\Pely\k + \bcomplpmp\k \cdot \Pcomplpmp\k + \bcomppr\k \cdot \Pcomppr\k ) & = & 0 \label{eq:bal_eq} 
\end{IEEEeqnarray}

Slack on fuel demand: 
\begin{IEEEeqnarray}{rCl}
	\mdotfueldemand\k & = & \mdotfuelmp\k + \zfuelmismatch\k \label{eq:slack_fuel} 
\end{IEEEeqnarray}

Box constraints: 
\begin{IEEEeqnarray}{rCl}
	\btildeelyon\k \cdot \Pelymin & \leq & \Pely\k \label{eq:b_tilde_1} \\ 
	\Pely\k & \leq & \btildeelyon\k \cdot \Pelymax \label{eq:b_tilde_2} 
\end{IEEEeqnarray}
Note that if the overload behavior is enabled, then $\Pelymax > \Pelynom$ and the constraints \eqref{eq:z_overload},~\eqref{eq:Eelyoverload_max} ensure that \Pelynom is exceeded only temporarily. 
If not, $\Pelymax = \Pelynom$. 

\begin{IEEEeqnarray}{rCcCl}
	\mlpmin & \leq & \mlp\k & \leq & \mlpmax \label{eq:m_lp_box} \\ 
	\mmpmin & \leq & \mmp\k & \leq & \mmpmax \label{eq:m_mp_box} 
\end{IEEEeqnarray}

Logical constraints for operation: 
\begin{IEEEeqnarray}{rCl}
	\bcomplpmp\k + \bcomppr\k & \leq & 1 \label{eq:bcomp_logic}
\end{IEEEeqnarray}

Constraint enforcing pressure recovery (pressure recovery must run for at least \tpr hours within a horizon where \bconsiderpr is set to 1: 
\begin{IEEEeqnarray}{rCl}
	\sum_{k=0}^{\Npred-1} \bconsiderpr\k \cdot \bcomppr\k \cdot \Tsampk & \geq & \tpr \label{eq:tpr}
\end{IEEEeqnarray}

\subsection{Startup Constraints}
For considering the startup, we introduce an auxiliary variable \btildeelyon (note the '$\sim$'). 
\belyon controls when we request to switch on (or off) the electrolyzer, 
and \btildeelyon is the actual availability signal, because it takes the electrolyzer approx. 15 minutes to warm up, before he can produce any H2. 
For example, if it takes the electrolyzer 2 timesteps to turn on, the signals can look like this: \\
$\belyon = [0, 1, 1, 1, 1] \rightarrow$ we switch on the ely in step 2 and then keep it on. \\
$\btildeelyon = [0, 0, 0, 1, 1] \rightarrow $ it takes 2 timesteps until power is available, \ie \\
$\Pely = [0, 0, 0, X, X]$. \\

This is realized by constraining \btildeelyon with logical AND-conditions on the previous \belyon signals. 
However, the corresponding number of steps varies throughout the prediction horizon, since the width of our time steps vary. 
Thus, this gets very tricky, and we need to calculate the corresponding number of steps in respect to the startup time. 

\subsubsection{Define $\nconsstartup$\,}
Additionally, to reduce the number of binary decision variables and because later in the horizon, the time steps are bigger than the actual start up constraint time, we do not consider the startup constraints in the entire horizon. 
Instead, all the following constraints are not used for $k = 0 \ldots \Npred-1$, but only for $k = 0 \ldots \nconsstartup$. 

With a start-up time of $\telystartup= 0.25\hours$, we consider the constraints only for the first 
\begin{IEEEeqnarray}{rCl}
	\nconsstartup & = & \argmax_i \Tsamp(i) \leq 2 \cdot \telystartup \label{eq:nconsstartup}
\end{IEEEeqnarray}
steps, where the factor of $2$ could be adjusted. 

\subsubsection{Determine the number of look back steps}
For every of the first $ n = 0, \ldots, ... \nconsstartup$ steps in the prediction horizon, we determine how many steps $\nlbpred(n)$ we have to look back within the prediction horizon; 
and how many steps $\nlbhist(n)$ into the history. 
Note that this is necessary due to both implementation and the varying time steps. 
Namely, we assume that the history of applied steps has the step width of $\Tsamp(0)$. 

%However, for the sake of readability, let us use $\nlbtotal(n) = \nlbpred(n) + \nlbhist(n)$. 
In the following, we use the notation $r\nk$, which in context of MPC usually refers to the predicted value of $r(k+n)$ at time step $k$. 
In addition, here a negative $n$ shall refer to a previous (historical) value. 

Then, at simulation step $k$, the additional constraints are 
%\begin{IEEEeqnarray}{rCl}
%	\btildeelyon\nk & = & \AND\left( 
%		\belyon(n|k), \belyon(n-1|k), \ldots, \belyon(n-\nlbtotal(n) |k) \right) 
%		\quad \forall~ n = 0,\,\ldots\,, \nconsstartup
%		\label{eq:constraints_btildeelyon} 
%\end{IEEEeqnarray}
%\red{or actually: }
\begin{IEEEeqnarray}{rCl}
	\btildeelyon\nk & = & \AND\bigg(
	\AND(
	\belyon(n|k), \belyon(n-1|k), \ldots, \belyon(n-\nlbpred(n) |k)  
	), 
	\label{eq:constraints_btildeelyon_nlbpred}
	\\ &&  
	\quad \quad \quad ~
	\OR\Big(   
	\AND ( \belyon(-1|k), ~\ldots~, \belyon(-\nlbhist(n) |k) ),~~
	\belyready(k)
	\Big)
	\bigg)
	\label{eq:constraints_btildeelyon_nlbhist}
	\\ &&  
	\quad \forall~ n = 0,\,\ldots\,, \nconsstartup. 
	\label{eq:constraints_btildeelyon_forall} 
\end{IEEEeqnarray}
Thereby, $\belyready(k)$ is a measured parameter which takes into account that the electrolyzer might have the status 'ready' even if we did not actively set $\belyon = 1$ in the past. 
Furthermore, $y = \AND(x_1,\,\ldots\,, x_z)$ denotes the logical and-function $y = x_1~\&~ \ldots~ \& ~x_z$, which is equivalent to the constraints 
%   n = len(xs)
%	expr = sum(xs) - n * y
%	return [0 <= expr, expr <= n - 1]
\begin{IEEEeqnarray}{rCl}
	0 & \leq  & \sum_{i=1}^{z} x_i - z \cdot y, \label{eq:and_constraint_1} \\
	\sum_{i=1}^{z} x_i - z \cdot y & \leq  & z - 1, \label{eq:and_constraint_2} 
\end{IEEEeqnarray}
and $y = \OR(x_1,\,\ldots\,, x_z)$ denotes the logical or-function $y = x_1~|~ \ldots~ | ~x_z$, which is equivalent to the constraints 
%   n = len(xs)
%	expr = n * y - cp.sum(xs)
%	return [0 <= expr, expr <= n - 1]
\begin{IEEEeqnarray}{rCl}
	0 & \leq  & z \cdot y - \sum_{i=1}^{z} x_i, \label{eq:or_constraint_1} \\
	z \cdot y - \sum_{i=1}^{z} x_i & \leq  & z - 1.  \label{eq:or_constraint_2} 
\end{IEEEeqnarray}
Note that if no historical lookback is necessary, \ie $\nlbhist(n) = 0$, then the $\OR(\cdot)$ term in \eqref{eq:constraints_btildeelyon_nlbhist} is dropped. 

For the rest of the horizon (beyond \nconsstartup), we do not distinguish between \belyon and \btildeelyon, \ie 
\begin{IEEEeqnarray}{rCl}
	\btildeelyon\nk & =  & \belyon\nk \quad \forall~ n = \nconsstartup+1,\,\ldots\,, \Npred-1 
	\label{eq:btildeelyon_after_ncons} 
\end{IEEEeqnarray}


\subsection{Overload Behavior}
The electrolyzer can be allowed to go in overload mode, \ie to exceed the nominal limit $\Pelynom = 225\kW$.
However, this can be done only for a limited amount of time. 
More precisely, this can be modeled as an \textit{energy buffer}, \Eelyovermax. 
\begin{IEEEeqnarray}{rCl}
	\zoverloadenergy(k) & \geq & \max\big( 0,~~ \Eelyover\k + \left( \Pely\k - \Pelynom \right) \cdot \Tsampk \big) \label{eq:zoverloadenergy}\\
	\Eelyover\kpo & = & \zoverloadenergy(k)   \label{eq:Eelyoverload} \\
	\Eelyover\k & \leq & \Eelyovermax \label{eq:Eelyoverload_max}
\end{IEEEeqnarray}
Note that we would actually want '$=$' in \eqref{eq:zoverloadenergy}. 
However, this would be a non-affine expression. 
Thus, we need to use $\geq$ and slightly punish the slack variable \zoverloadenergy, see Section~\ref{subsubsec:further_slack_costs}. 


\subsection{1-Dimensional Efficiency Maps (piece-wise linear approximation)}

The mapping $\mdotely = f_\g{ely}(\Pely)$ is formulated as a one-dimensional piece-wise linear approximation (PWLA), as illustrated in \figref{fig:one_dim_pwla}. 

\begin{figure}[htb]%[h]
	%	\captionsetup{belowskip=-20pt,aboveskip=0pt}
	\centering
	\textbf{\small One-Dimensional Piecewise Linear Approximation}\par
	\includegraphics[width=0.8\linewidth]{figs/one-dim-pwla.png}	
	\caption{
		Illustration and summary of the one-dimensional PWLA. 
	}
	\label{fig:one_dim_pwla}
\end{figure}

Currently, it is implemented with 3 grid points, taken from a different electrolyzer, since HTEC has yet not provided the efficiency curve. 
These are: $\Pelysamples = (0, 60, 350)\,\kW,~~ \mdotelysamples = (0, 1.01, 4.71)\,\frac{\kg}{\hours} $. 
Using additional continuous variables \lambdaelyi and binary variables \deltaelyi, the PWLA is realized by:

\begin{IEEEeqnarray}{c}
	\Pely\k 		= \sum_{i=1}^{3} \lambdaelyi\k \cdot \Pelysamplesi, \\
	\mdotely\k 		= \sum_{i=1}^{3} \lambdaelyi\k \cdot \mdotelysamplesi, \\
	\sum_{i=1}^{3} \lambdaelyi\k = 1, \\
	0 \leq \lambdaelyi\k \forall i = 1, \ldots, 3, \\
	\sum_{i=1}^{3} \deltaelyi\k = 1, \\
	\lambdaelyi\k \leq \deltaelyimo\k + \deltaelyi\k. 
\end{IEEEeqnarray}

Furthermore, the compressor's flow, \ie H2 output in $\nicefrac{\kg}{\hours}$, also depends on the input pressure. 
Note that, actually, it also depends on the output pressure. 
However, the dependency on the output pressure is small and can be neglected for the control purpose. 
Thus, it is sufficient to again use a one-dimensional PWLA, using the sample points 
$\mlpsamples = (0, 20, 90)\,\barpressure,~~ \mdotlpmpsamples = (0.2, 4.2, 18.0)\,\frac{\kg}{\hours}$. 
It is described by: 

\begin{IEEEeqnarray}{c}
	\mlp\k 		= \sum_{i=1}^{3} \lambdalpmpi\k \cdot \mlpsamplesi, \\
	\mdotlpmp\k 		= \sum_{i=1}^{3} \lambdalpmpi\k \cdot \mdotlpmpsamplesi, \\
	\sum_{i=1}^{3} \lambdalpmpi\k = 1, \\
	0 \leq \lambdalpmpi\k \forall i = 1, \ldots, 3, \\
	\sum_{i=1}^{3} \deltalpmpi\k = 1, \\
	\lambdalpmpi\k \leq \deltalpmpimo\k + \deltalpmpi\k. 
\end{IEEEeqnarray}

\subsection{2-Dimensional Efficiency Maps}
The compressor's power cannot be modulated, \ie it is either running or not. 
Thereby, both the compressor's power consumption \Pcomp significantly depends on both the input and output pressure. 
Thus, a one-dimensional PWLA is not sufficient. 
Instead, we use the triangle method for a two-dimensional PWLA, see \cite{dambrosio2010piecewise}. 

Assume the mapping $(x, y) \rightarrow f(x,y)$ with \nx grid points in $x$-direction and \my grid points in $y$-direction. 
The general idea is then to split the grid of the $\nx \cdot \my$ base points into triangles. 
Consider $\xbar \in [\xip, \xipo]$ and $\ybar \in [\yjp, \yjpo]$. 
Then, the rectangle defined by $[\xip, \xipo]$ and $[\yjp, \yjpo]$ is split into two triangles, as illustrated in \figref{fig:two_dim_pwla_triangle}. 
$(\xbar, \ybar)$ can then be expressed as a convex combination of either 
$(\xip, \yjp),~ (\xipo, \yjpo)$ and $(\xip, \yjpo)$, or of 
$(\xip, \yjp),~ (\xipo, \yjpo)$ and $(\xipo, \yjp)$, 
depending on whether $(\xbar, \ybar)$ lies in the upper or lower triangle, respectively. 
Namely, for every grid point $(\xip, \yjp)$, an additional continuous variable $\alphaij \in [0,1]$ is introduced. 
Then, $(\xbar, \ybar)$ is expressed by a convex combination of all \alphaij, \ie 
\begin{IEEEeqnarray}{rCl}
	x &=& \sum_{i=1}^{\nx} \sum_{j=1}^{\my} \alphaij \xip \label{eq:x_alphaij}, \\
	y &=& \sum_{i=1}^{\nx} \sum_{j=1}^{\my} \alphaij \yjp \label{eq:y_alphaij}. 
\end{IEEEeqnarray}
To determine in which triangle $(\xbar, \ybar)$ lies, we introduce $2 \cdot \nx \cdot \my$ binary variables \huij and \hlij, which indicate whether $(\xbar, \ybar)$ is in the upper or lower triangle within the rectangle spanned by $(\xip, \yjp),~ (\xipo, \yjpo)$, $(\xip, \yjpo)$ and $(\xipo, \yjp)$. 
For further details, refer to \cite{dambrosio2010piecewise}. 


%\begin{IEEEeqnarray}{c}
%	\sum_{i=1}^{\nx-1} \sum_{j=1}^{\my-1} (\huij + \hlij) = 1 \label{eq:2dim_pwla_1}, \\
%\end{IEEEeqnarray}


\begin{figure}[htb]%[h]
	%	\captionsetup{belowskip=-20pt,aboveskip=0pt}
	\centering
	\textbf{\small Triangle Method: Two-Dimensional Piecewise Linear Approximation}\par
	
	\includegraphics[width=0.4\linewidth]{figs/two_dim_pwla_triangle.png}	
	\caption{
		Illustration of the triangle method for a two-dimensional PWLA. 
		Source: \cite{dambrosio2010piecewise}
	}
	\label{fig:two_dim_pwla_triangle}
\end{figure}

\subsection{Soft Constraints}

For both the LP and MP tanks, 
higher lower limits ($\mlpminsoft > \mlpmin, ~ \mmpminsoft > \mmpmin$)  and 
lower  upper limits ($\mlpmaxsoft < \mlpmax, ~ \mmpmaxsoft < \mmpmax$)  
are enforced by using 'soft constraints. 
However, we do not use a slack variable on the box constraints of \mlp and \mmp, but we only punish deviations with a high value in the objective function. 
The corresponding cost terms \Jsclp and \Jscmp are described in Section~\ref{subsubsec:operational_costs}


\subsection{Objective Function(s)}



\subsubsection{Monetary Costs}
For the grid costs, different prices \cgridbuy for buying and \cgridsell for selling are assumed. 
To formulate them not only convex, but also following Disciplined Parametrized Programming\footnote{See \url{https://www.cvxpy.org/tutorial/advanced/index.html\#disciplined-parametrized-programming}} (DPP) rules, we use $\cgriddiff = \cgridbuy - \cgridsell > 0$: 
\begin{IEEEeqnarray}{rCl}
	\Jmongrid(k) & = & 
	\sumnNp \big(  
	\cgriddiff\nk \cdot \max(0,~ \Pgrid\nk) + \cgridsell\nk \cdot \Pgrid\nk  
	\big) \cdot \Tsamp\nk
	\label{eq:Jmongrid}
\end{IEEEeqnarray}
Note that we currently use only constant values for \cgridbuy and \cgridsell, but they are treated as parameters which can change every time step. 

The peak costs are calculated as follows:
\begin{IEEEeqnarray}{rCl}
	\Jmonpeak\k  & = & \max\left( 
	\max_{k=0,\ldots, \Np-1} \Big(0,~ \cgridpeak \cdot \Pgrid\nk - \Jmonpeakprev\k \Big) 
	\right), 
	\label{eq:Jmonpeak}  
\end{IEEEeqnarray}
where \Jmonpeakprev is implemented as a parameter which is calculated before at each time step. 
It denotes the already occurred peak costs. 

Water costs for the electrolysis are given by: 
\begin{IEEEeqnarray}{rCl}
	\Jmonwater(k) & = & 
	\sumnNp \big( \cwater \cdot \mdotely\nk \big) \cdot \Tsamp\nk
	\label{eq:Jmonwater}
\end{IEEEeqnarray}

%%% The following is only if H2-> Heat is used, here not assumed: %%% 

%Furthermore, if H2 to heat is used, the monetary costs for gas are: 
%\begin{IEEEeqnarray}{rCl}
%	\Jmongas(k) & = & 
%		\sumnNp \big( \cgas \cdot \Qgas\nk \big) \cdot \Tsamp\nk
%		\label{eq:Jmongas}
%\end{IEEEeqnarray}

The total monetary costs are then 
\begin{IEEEeqnarray}{rCl}
	\Jmontotal(k) & = & \Jmongrid\k + \Jmonpeak\k + \Jmonwater\k. 
	\label{eq:Jmontotal}
\end{IEEEeqnarray}

\subsubsection{Operational Costs}
\label{subsubsec:operational_costs}

The tighter limits on both the LP and MP are enforced by: 
\begin{IEEEeqnarray}{rCl}
	\Jsclp\k & = & 
	10 \cdot \left( 
	\sumnNppo \max\left( 0,~ \mlpminsoft - \mlp\nk \right) +
	\sumnNppo \max\left( 0,~ \mlp\nk - \mlpmaxsoft \right)
	\right),   
	\label{eq:sc_lp} \\
	\Jscmp\k & = & 
	100 \cdot \left( 
	\sumnNppo \max\left( 0,~ \mmpminsoft - \mmp\nk \right) + 
	\sumnNppo \max\left( 0,~ \mmp\nk - \mmpmaxsoft \right)
	\right).    
	\label{eq:sc_mp} 
\end{IEEEeqnarray}

Furthermore, we punish every startup of the electrolyzer with a constant \cstartup: 
\begin{IEEEeqnarray}{rCl}
	\Jstartup(k) & = &  \sumnNp \max\big(0, ~\cstartup \cdot \toggleonoff\nk \big), \label{eq:Jstartup} \\
	\toggleonoff(k) & = & \belyon(k) - \belyon(k-1) \label{eq:Jstartup_2}
\end{IEEEeqnarray}

\subsubsection{User Satisfaction}
To enforce that any fuel demand is satisfied as much as possible, we punish the mismatch slack variable \zfuelmismatch from \eqref{eq:slack_fuel} strongly, \ie 
\begin{IEEEeqnarray}{rCl}
	\Juser(k) & = &  \cfueldemandmis \sumnNp \zfuelmismatch\nk \cdot \Tsamp\nk, \label{eq:Juser} 
\end{IEEEeqnarray}
with $\cfueldemandmis = 20\,\nicefrac{\meuro}{\kg}$. 

\subsubsection{\CO Emissions}
We punish \CO emissions separately, \ie 
\begin{IEEEeqnarray}{rCl}
	\Jco(k) & = &  \sumnNp \big(
	\cgridco \cdot \max(0,~ \Pgrid\nk) 
	%		+ \cgasco \cdot \Qgas\nk   % USE ONLY IF H2 -> HEAT IS ACTIVATED 
	\big) \cdot \Tsamp\nk, 
	\label{eq:Jco} 
\end{IEEEeqnarray}

\subsubsection{Further Slack Costs}
\label{subsubsec:further_slack_costs}
To ensure that \zoverloadenergy from \eqref{eq:zoverloadenergy} is not unnecessarily high, we slightly punish it with 
\begin{IEEEeqnarray}{rCl}
	\Jslack(k) & = &  10^{-3} \cdot \sumnNp \zoverloadenergy\nk. \label{eq:Jslack} 
\end{IEEEeqnarray}
